On Design and Implementation of the Distributed Modular Audio Recognition Framework: Requirements and Specification Design Document

We present the requirements and design specification of the open-source Distributed Modular Audio Recognition Framework (DMARF), a distributed extension of MARF. The distributed version aggregates a number of distributed technologies (e.g. Java RMI, CORBA, Web Services) in a pluggable and modular model along with the provision of advanced distributed systems algorithms. We outline the associated challenges incurred during the design and implementation as well as overall specification of the project and its advantages and limitations.

==> date.tex <==
Thu  1 May 2008 11:54:44 EDT

